Aportes para el cumplimiento del Reglamento (UE) 2024/1689 en rob\'otica y sistemas aut\'onomos

Cybersecurity in robotics stands out as a key aspect within Regulation (EU) 2024/1689, also known as the Artificial Intelligence Act, which establishes specific guidelines for intelligent and automated systems. A fundamental distinction in this regulatory framework is the difference between robots with Artificial Intelligence (AI) and those that operate through automation systems without AI, since the former are subject to stricter security requirements due to their learning and autonomy capabilities. This work analyzes cybersecurity tools applicable to advanced robotic systems, with special emphasis on the protection of knowledge bases in cognitive architectures. Furthermore, a list of basic tools is proposed to guarantee the security, integrity, and resilience of these systems, and a practical case is presented, focused on the analysis of robot knowledge management, where ten evaluation criteria are defined to ensure compliance with the regulation and reduce risks in human-robot interaction (HRI) environments.

==> ComparacionDeHerramientas.tex <==

\section{Comparación de las Herramientas}

Para evaluar las herramientas de ciberseguridad en robótica de acuerdo con este reglamento, se han identificado varios temas clave, los cuales se describen a continuación:

\begin{itemize}
    \item \textbf{Evaluación de Riesgos}: Analizar los riesgos específicos asociados a diferentes tipos de robots, adaptando las herramientas de ciberseguridad a estos riesgos.
    \item \textbf{Medidas de Protección de Datos}: Implementar protocolos que garanticen la privacidad y seguridad de los datos procesados por los robots.
    \item \textbf{Actualizaciones y Parches de Seguridad}: Evaluar la frecuencia y eficacia de las actualizaciones de seguridad y parches aplicados.
    \item \textbf{Resiliencia ante Ciberataques}: Comprobar la capacidad de los robots para resistir y recuperarse de ataques cibernéticos, incluyendo pruebas de penetración y simulaciones de ataques.
    \item \textbf{Cumplimiento de Normas y Estándares}: Asegurar que las herramientas de ciberseguridad estén alineadas con los estándares y normativas europeas e internacionales.
    \item \textbf{Seguridad en Comunicaciones}: Proteger las comunicaciones entre robots y otros sistemas, utilizando cifrado de datos y medidas contra interceptaciones.
    \item \textbf{Gestión de Vulnerabilidades}: Establecer procesos para la identificación, evaluación y mitigación de vulnerabilidades en los sistemas de los robots.
    \item \textbf{Plan de Respuesta a Incidentes}: Implementar procedimientos para la detección, análisis y respuesta ante incidentes de seguridad.
    \item \textbf{Auditorías y Supervisión}: Realizar auditorías y supervisión continua de las medidas de ciberseguridad implementadas en los robots.
\end{itemize}


\subsection{Descripción de la Comparación de las Herramientas}

A continuación, se detallan los aspectos evaluados en cada herramienta de ciberseguridad, junto con ejemplos específicos aplicables en entornos de \textit{ROS/ROS 2}.

\subsubsection{Sistemas de Detección de Intrusiones (IDS) y Prevención (IPS)}
\begin{itemize}
    \item \textbf{Evaluación de Riesgos}: Detectan y previenen intrusiones en la red, proporcionando análisis de riesgos en tiempo real.
    \item \textbf{Medidas de Protección de Datos}: Ayudan a proteger los datos mediante la detección y prevención de accesos no autorizados.
    \item \textbf{Actualizaciones y Parches de Seguridad}: No aplican directamente parches, pero pueden complementarse con otras soluciones.
    \item \textbf{Resiliencia ante Ciberataques}: Mejoran la capacidad de respuesta ante amenazas al detectar ataques en tiempo real.
    \item \textbf{Cumplimiento de Normas y Estándares}: Utilizados para cumplir con normativas de seguridad de redes.
    \item \textbf{Seguridad en Comunicaciones}: Protegen la red contra ataques de interceptación y manipulación de tráfico.
    \item \textbf{Gestión de Vulnerabilidades}: Identifican vulnerabilidades a través de patrones de tráfico sospechosos.
    \item \textbf{Plan de Respuesta a Incidentes}: Permiten detectar y mitigar incidentes de seguridad rápidamente.
    \item \textbf{Auditorías y Supervisión}: Proporcionan registros detallados del tráfico de red y eventos de seguridad.

    \item         \textit{Ejemplo General}: Snort, Suricata.

\textit{Ejemplo}: \textbf{Zeek} (IDS de código abierto que se puede integrar con ROS 2 para monitorear tráfico de red en robots).
\end{itemize}

\subsubsection{Firewall de Próxima Generación (NGFW)}
\begin{itemize}
    \item \textbf{Evaluación de Riesgos}: Analizan y controlan el tráfico de red, previniendo amenazas.
    \item \textbf{Medidas de Protección de Datos}: Filtran accesos no autorizados para proteger la integridad de los datos.
    \item \textbf{Actualizaciones y Parches de Seguridad}: Reciben actualizaciones, pero no son herramientas específicas para la gestión de parches.
    \item \textbf{Resiliencia ante Ciberataques}: Detectan y bloquean ataques avanzados en tiempo real.
    \item \textbf{Cumplimiento de Normas y Estándares}: Implementan políticas de seguridad que garantizan el cumplimiento de normativas.
    \item \textbf{Seguridad en Comunicaciones}: Aseguran la protección del tráfico mediante filtrado y análisis de paquetes.
    \item \textbf{Gestión de Vulnerabilidades}: Identifican amenazas dentro del tráfico de red.
    \item \textbf{Plan de Respuesta a Incidentes}: Detectan y responden a eventos de seguridad en la red.
    \item \textbf{Auditorías y Supervisión}: Permiten analizar logs y generar informes de tráfico y ataques.
    \item \textit{Ejemplo}: \textbf{Palo Alto Networks} (usado para la seguridad de infraestructuras que soportan ROS 2 en la nube).
      \textit{Ejemplo}: Palo Alto Networks, Fortinet.
\end{itemize}

\subsubsection{Soluciones de Gestión de Información y Eventos de Seguridad (SIEM)}
\begin{itemize}
    \item \textbf{Evaluación de Riesgos}: Recopilan y analizan eventos de seguridad para detectar riesgos.
    \item \textbf{Medidas de Protección de Datos}: Monitorean y protegen eventos relacionados con el acceso a datos.
    \item \textbf{Actualizaciones y Parches de Seguridad}: No aplican parches directamente, pero pueden detectar vulnerabilidades que requieren actualizaciones.
    \item \textbf{Resiliencia ante Ciberataques}: Detectan patrones anómalos que podrían indicar ataques cibernéticos.
    \item \textbf{Cumplimiento de Normas y Estándares}: Ayudan a cumplir normativas mediante informes detallados de eventos.
    \item \textbf{Seguridad en Comunicaciones}: Supervisan el tráfico de red en busca de amenazas relacionadas con la comunicación.
    \item \textbf{Gestión de Vulnerabilidades}: Identifican brechas de seguridad mediante análisis de eventos.
    \item \textbf{Plan de Respuesta a Incidentes}: Permiten detectar y responder a amenazas en tiempo real.
    \item \textbf{Auditorías y Supervisión}: Generan informes de seguridad detallados.
    \item \textit{Ejemplo}: \textbf{Wazuh} (plataforma SIEM de código abierto compatible con ROS 2 para monitoreo de seguridad en sistemas distribuidos).
      \textit{Ejemplo}: Splunk, IBM QRadar.
\end{itemize}

%La siguiente subsection estaba repetida por lo que la he eliminado


\subsubsection{Autenticación Fuerte y Control de Acceso}
\begin{itemize}
    \item \textbf{Evaluación de Riesgos}: Controlan el acceso a sistemas y datos, minimizando riesgos de accesos indebidos.
    \item \textbf{Medidas de Protección de Datos}: Garantizan que solo usuarios autorizados accedan a información sensible.
    \item \textbf{Actualizaciones y Parches de Seguridad}: No son herramientas específicas para la gestión de parches.
    \item \textbf{Resiliencia ante Ciberataques}: Reducen el riesgo de ataques por suplantación de identidad o accesos no autorizados.
    \item \textbf{Cumplimiento de Normas y Estándares}: Facilitan el cumplimiento de normativas de autenticación y acceso.
    \item \textbf{Seguridad en Comunicaciones}: Protegen las credenciales de los usuarios en la comunicación con los sistemas.
    \item \textbf{Gestión de Vulnerabilidades}: Identifican y previenen accesos indebidos a recursos críticos.
    \item \textbf{Plan de Respuesta a Incidentes}: Detectan y bloquean accesos sospechosos en tiempo real.
    \item \textbf{Auditorías y Supervisión}: Registran intentos de acceso y generan reportes de autenticación.
    \item \textit{Ejemplo}: \textbf{SROS} (implementado en ROS 2 para autenticación segura y control de acceso mediante políticas de seguridad).
\end{itemize}

\subsubsection{Segmentación de Redes}
\begin{itemize}
    \item \textbf{Evaluación de Riesgos}: Permite limitar la propagación de amenazas al segmentar la red en diferentes zonas de seguridad.
    \item \textbf{Medidas de Protección de Datos}: Controla y restringe el acceso a datos sensibles dentro de segmentos de red.
    \item \textbf{Actualizaciones y Parches de Seguridad}: No son herramientas específicas para la gestión de parches.
    \item \textbf{Resiliencia ante Ciberataques}: Minimiza el impacto de ataques aislando zonas comprometidas.
    \item \textbf{Cumplimiento de Normas y Estándares}: Implementa políticas de segmentación conforme a normativas de seguridad.
    \item \textbf{Seguridad en Comunicaciones}: Protege las comunicaciones entre segmentos, evitando accesos no autorizados.
    \item \textbf{Gestión de Vulnerabilidades}: Facilita la contención de vulnerabilidades en zonas críticas.
    \item \textbf{Plan de Respuesta a Incidentes}: Ayuda a restringir y contener incidentes de seguridad.
    \item \textbf{Auditorías y Supervisión}: Proporciona visibilidad del tráfico y accesos dentro de la red segmentada.
    \item \textit{Ejemplo}: \textbf{Cisco TrustSec} (implementado en infraestructuras para proteger redes industriales y robóticas).
\end{itemize}

\subsubsection{Sistemas de Gestión de Parches}
\begin{itemize}
    \item \textbf{Evaluación de Riesgos}: Identifican sistemas desactualizados y evalúan su exposición a vulnerabilidades.
    \item \textbf{Medidas de Protección de Datos}: No son herramientas específicas para la protección de datos.
    \item \textbf{Actualizaciones y Parches de Seguridad}: Aplican y gestionan parches de seguridad de manera automatizada.
    \item \textbf{Resiliencia ante Ciberataques}: Reducen la probabilidad de ataques explotando vulnerabilidades conocidas.
    \item \textbf{Cumplimiento de Normas y Estándares}: Facilitan la actualización de sistemas según normativas de seguridad.
    \item \textbf{Seguridad en Comunicaciones}: No tienen un enfoque específico en comunicaciones seguras.
    \item \textbf{Gestión de Vulnerabilidades}: Identifican y priorizan vulnerabilidades en software y sistemas.
    \item \textbf{Plan de Respuesta a Incidentes}: No están diseñados para la respuesta activa ante incidentes.
    \item \textbf{Auditorías y Supervisión}: Registran el estado de actualización de sistemas y generan informes.
    \item \textit{Ejemplo}: \textbf{Canonical Livepatch} (permite la aplicación de parches en tiempo real en sistemas basados en Ubuntu, utilizado en entornos ROS 2).
\end{itemize}

\subsubsection{Monitorización y Detección de Amenazas}
\begin{itemize}
    \item \textbf{Evaluación de Riesgos}: Permiten identificar riesgos y amenazas en tiempo real mediante el análisis de tráfico y eventos.
    \item \textbf{Medidas de Protección de Datos}: Detectan accesos no autorizados y anomalías en el tratamiento de datos.
    \item \textbf{Actualizaciones y Parches de Seguridad}: No son herramientas específicas para la gestión de parches.
    \item \textbf{Resiliencia ante Ciberataques}: Detectan ataques en tiempo real y permiten responder rápidamente.
    \item \textbf{Cumplimiento de Normas y Estándares}: Facilitan el monitoreo continuo para asegurar el cumplimiento normativo.
    \item \textbf{Seguridad en Comunicaciones}: Analizan el tráfico de red en busca de patrones sospechosos.
    \item \textbf{Gestión de Vulnerabilidades}: Ayudan a identificar y remediar vulnerabilidades activas.
    \item \textbf{Plan de Respuesta a Incidentes}: Permiten la detección temprana y generación de alertas de seguridad.
    \item \textbf{Auditorías y Supervisión}: Proporcionan informes detallados sobre eventos de seguridad.
    \item \textit{Ejemplo}: \textbf{Falco} (herramienta de monitorización y detección de amenazas para contenedores y sistemas ROS 2).
\end{itemize}

\subsubsection{Soluciones de Respuesta y Recuperación ante Incidentes}
\begin{itemize}
    \item \textbf{Evaluación de Riesgos}: Evalúan el impacto de un incidente y facilitan la gestión de la recuperación.
    \item \textbf{Medidas de Protección de Datos}: Implementan protocolos para la contención y recuperación de datos comprometidos.
    \item \textbf{Actualizaciones y Parches de Seguridad}: No son herramientas específicas para la gestión de parches, pero pueden sugerir acciones correctivas.
    \item \textbf{Resiliencia ante Ciberataques}: Ayudan a restaurar operaciones tras un incidente, minimizando daños.
    \item \textbf{Cumplimiento de Normas y Estándares}: Documentan incidentes y aseguran que las respuestas cumplan con normativas.
    \item \textbf{Seguridad en Comunicaciones}: Protegen la integridad de las comunicaciones durante y después de un incidente.
    \item \textbf{Gestión de Vulnerabilidades}: Identifican y mitigan vulnerabilidades explotadas en ataques recientes.
    \item \textbf{Plan de Respuesta a Incidentes}: Proporcionan guías y herramientas para la gestión eficiente de incidentes.
    \item \textbf{Auditorías y Supervisión}: Permiten documentar y analizar incidentes para mejorar estrategias futuras.
    \item \textit{Ejemplo}: \textbf{TheHive} (plataforma de respuesta ante incidentes de código abierto que puede integrarse en infraestructuras de ROS 2).
\end{itemize}


\subsubsection{Seguridad en Comunicaciones}
\begin{itemize}
    \item \textbf{Evaluación de Riesgos}: Asegura la protección de las comunicaciones entre nodos y sistemas distribuidos.
    \item \textbf{Medidas de Protección de Datos}: Cifra la transmisión de datos para evitar accesos no autorizados.
    \item \textbf{Actualizaciones y Parches de Seguridad}: No son herramientas específicas para la gestión de parches.
    \item \textbf{Resiliencia ante Ciberataques}: Reduce el riesgo de ataques de interceptación y manipulación de mensajes.
    \item \textbf{Cumplimiento de Normas y Estándares}: Implementa protocolos de cifrado alineados con estándares de seguridad.
    \item \textbf{Gestión de Vulnerabilidades}: Identifica y mitiga vulnerabilidades en la comunicación entre nodos.
    \item \textbf{Plan de Respuesta a Incidentes}: Detecta y bloquea intentos de manipulación de tráfico en la red.
    \item \textbf{Auditorías y Supervisión}: Registra eventos de comunicación para detectar anomalías o accesos indebidos.
    \item \textit{Ejemplo}: \textbf{SROS} (utiliza TLS y cifrado de datos en ROS 2 para proteger las comunicaciones).
\end{itemize}

